Iterative beam search algorithms for the permutation flowshop

We study an iterative beam search algorithm for the permutation flowshop (makespan and flowtime minimization). This algorithm combines branching strategies inspired by recent branch-and-bounds and a guidance strategy inspired by the LR heuristic. It obtains competitive results, reports many new-best-so-far solutions on the VFR benchmark (makespan minimization) and the Taillard benchmark (flowtime minimization) without using any NEH-based branching or iterative-greedy strategy. The source code is available at: https://gitlab.com/librallu/cats-pfsp.

==> 1_makespan.tex <==
{\footnotesize\selectfont
\begin{tabular}{|l|l|l|}
    \hline
        & best	& IBS1	\\
    \hline
    100\_20\_1	& 6.173	& \textbf{6.172}	\\
    100\_20\_2	& 6.267	& 6.306	\\
    100\_20\_3	& 6.221	& 6.231	\\
    100\_20\_4	& 6.227	& 6.268	\\
    100\_20\_5	& 6.264	& 6.330	\\
    100\_20\_6	& 6.285	& 6.333	\\
    100\_20\_7	& 6.401	& 6.409	\\
    100\_20\_8	& 6.074	& 6.083	\\
    100\_20\_9	& 6.328	& 6.426	\\
    100\_20\_10	& 6.125	& 6.167	\\
    100\_40\_1	& 7.846	& 8.010	\\
    100\_40\_2	& 7.976	& 8.091	\\
    100\_40\_3	& 7.894	& 8.018	\\
    100\_40\_4	& 7.913	& 8.154	\\
    100\_40\_5	& 7.997	& 8.108	\\
    100\_40\_6	& 7.993	& 8.279	\\
    100\_40\_7	& 7.980	& 8.344	\\
    100\_40\_8	& 7.957	& 8.122	\\
    100\_40\_9	& 7.888	& 7.987	\\
    100\_40\_10	& 7.917	& 8.036	\\
    100\_60\_1	& 9.353	& 9.757	\\
    100\_60\_2	& 9.567	& 9.738	\\
    100\_60\_3	& 9.349	& 9.656	\\
    100\_60\_4	& 9.403	& 9.613	\\
    100\_60\_5	& 9.431	& 9.966	\\
    100\_60\_6	& 9.630	& 10.016	\\
    100\_60\_7	& 9.346	& 9.654	\\
    100\_60\_8	& 9.523	& 9.843	\\
    100\_60\_9	& 9.488	& 10.070	\\
    100\_60\_10	& 9.572	& 9.829	\\
    200\_20\_1	& 11.272	& 12.213	\\
    200\_20\_2	& 11.240	& 11.444	\\
    200\_20\_3	& 11.294	& 11.328	\\
    200\_20\_4	& 11.188	& 11.265	\\
    200\_20\_5	& 11.143	& 11.242	\\
    200\_20\_6	& 11.310	& 11.428	\\
    200\_20\_7	& 11.365	& 11.437	\\
    200\_20\_8	& 11.128	& 11.279	\\
    200\_20\_9	& 11.091	& 11.285	\\
    200\_20\_10	& 11.294	& 11.366	\\
    200\_40\_1	& 13.124	& 13.139	\\
    200\_40\_2	& 13.049	& 13.131	\\
    200\_40\_3	& 13.222	& 13.228	\\
    200\_40\_4	& 13.163	& 13.232	\\
    200\_40\_5	& 12.974	& 12.997	\\
    200\_40\_6	& 13.061	& 13.134	\\
    200\_40\_7	& 13.220	& 13.296	\\
    200\_40\_8	& 13.132	& \textbf{13.123}	\\
    200\_40\_9	& 13.033	& 13.051	\\
    200\_40\_10	& 13.146	& \textbf{13.114}	\\
    200\_60\_1	& 14.906	& 15.029	\\
    200\_60\_2	& 14.909	& 15.236	\\
    200\_60\_3	& 15.134	& 15.598	\\
    200\_60\_4	& 14.968	& 15.376	\\
    200\_60\_5	& 15.042	& 15.414	\\
    200\_60\_6	& 14.996	& 15.101	\\
    200\_60\_7	& 15.006	& 15.180	\\
    200\_60\_8	& 14.894	& 15.170	\\
    200\_60\_9	& 14.925	& 15.167	\\
    200\_60\_10	& 14.908	& 15.203	\\
    \hline
    \end{tabular}
    \begin{tabular}{|l|l|l|}
    \hline
        & best	& IBS1	\\
    \hline
    300\_20\_1	& 16.089	& 16.278	\\
    300\_20\_2	& 16.483	& 16.735	\\
    300\_20\_3	& 16.129	& 16.340	\\
    300\_20\_4	& 16.168	& 16.368	\\
    300\_20\_5	& 16.307	& 16.524	\\
    300\_20\_6	& 16.095	& 16.292	\\
    300\_20\_7	& 16.244	& 16.705	\\
    300\_20\_8	& 16.369	& 16.487	\\
    300\_20\_9	& 16.324	& 16.473	\\
    300\_20\_10	& 16.798	& 17.010	\\
    300\_40\_1	& 18.199	& \textbf{18.059}	\\
    300\_40\_2	& 18.373	& \textbf{18.218}	\\
    300\_40\_3	& 18.348	& \textbf{18.242}	\\
    300\_40\_4	& 18.227	& \textbf{18.095}	\\
    300\_40\_5	& 18.343	& \textbf{18.195}	\\
    300\_40\_6	& 18.340	& \textbf{18.177}	\\
    300\_40\_7	& 18.396	& \textbf{18.202}	\\
    300\_40\_8	& 18.290	& \textbf{18.187}	\\
    300\_40\_9	& 18.261	& \textbf{18.093}	\\
    300\_40\_10	& 18.286	& \textbf{18.132}	\\
    300\_60\_1	& 20.483	& 20.662	\\
    300\_60\_2	& 20.249	& 20.444	\\
    300\_60\_3	& 20.328	& 20.468	\\
    300\_60\_4	& 20.293	& 20.564	\\
    300\_60\_5	& 20.200	& 20.235	\\
    300\_60\_6	& 20.280	& 20.400	\\
    300\_60\_7	& 20.358	& 20.638	\\
    300\_60\_8	& 20.319	& 20.647	\\
    300\_60\_9	& 20.405	& 20.503	\\
    300\_60\_10	& 20.385	& 20.458	\\
    400\_20\_1	& 21.042	& 21.383	\\
    400\_20\_2	& 21.411	& 21.611	\\
    400\_20\_3	& 21.428	& 21.979	\\
    400\_20\_4	& 21.237	& 21.432	\\
    400\_20\_5	& 21.528	& 21.666	\\
    400\_20\_6	& 21.188	& 21.311	\\
    400\_20\_7	& 21.599	& 21.825	\\
    400\_20\_8	& 21.264	& 21.478	\\
    400\_20\_9	& 21.293	& 21.480	\\
    400\_20\_10	& 21.526	& 21.705	\\
    400\_40\_1	& 23.393	& \textbf{23.159}	\\
    400\_40\_2	& 23.380	& \textbf{23.055}	\\
    400\_40\_3	& 23.467	& \textbf{23.258}	\\
    400\_40\_4	& 23.269	& \textbf{22.896}	\\
    400\_40\_5	& 23.213	& \textbf{22.984}	\\
    400\_40\_6	& 23.298	& \textbf{23.103}	\\
    400\_40\_7	& 23.415	& \textbf{23.197}	\\
    400\_40\_8	& 23.290	& \textbf{23.149}	\\
    400\_40\_9	& 23.424	& \textbf{23.322}	\\
    400\_40\_10	& 23.606	& \textbf{23.362}	\\
    400\_60\_1	& 25.395	& \textbf{25.359}	\\
    400\_60\_2	& 25.549	& 25.636	\\
    400\_60\_3	& 25.707	& \textbf{25.658}	\\
    400\_60\_4	& 25.638	& 25.797	\\
    400\_60\_5	& 25.669	& 25.788	\\
    400\_60\_6	& 25.407	& 25.473	\\
    400\_60\_7	& 25.415	& 25.434	\\
    400\_60\_8	& 25.603	& \textbf{25.509}	\\
    400\_60\_9	& 25.673	& 25.731	\\
    400\_60\_10	& 25.658	& 25.747	\\
    \hline
    \end{tabular}
    \begin{tabular}{|l|l|l|}
        \hline
            & best	& IBS1	\\
        \hline
        500\_20\_1	& 26.374	& 26.656	\\
        500\_20\_2	& 26.641	& 26.862	\\
        500\_20\_3	& 26.359	& 26.593	\\
        500\_20\_4	& 26.080	& 26.295	\\
        500\_20\_5	& 26.759	& 27.169	\\
        500\_20\_6	& 26.411	& 26.544	\\
        500\_20\_7	& 26.409	& 26.723	\\
        500\_20\_8	& 26.305	& 26.559	\\
        500\_20\_9	& 26.430	& 26.719	\\
        500\_20\_10	& 26.034	& 26.302	\\
        500\_40\_1	& 28.402	& \textbf{28.183}	\\
        500\_40\_2	& 28.613	& \textbf{28.310}	\\
        500\_40\_3	& 28.526	& \textbf{28.401}	\\
        500\_40\_4	& 28.615	& \textbf{28.378}	\\
        500\_40\_5	& 28.579	& \textbf{28.289}	\\
        500\_40\_6	& 28.432	& \textbf{28.138}	\\
        500\_40\_7	& 28.553	& \textbf{28.307}	\\
        500\_40\_8	& 28.488	& \textbf{28.299}	\\
        500\_40\_9	& 28.640	& \textbf{28.407}	\\
        500\_40\_10	& 28.644	& \textbf{28.318}	\\
        500\_60\_1	& 30.682	& \textbf{30.491}	\\
        500\_60\_2	& 30.664	& \textbf{30.532}	\\
        500\_60\_3	& 30.852	& \textbf{30.671}	\\
        500\_60\_4	& 30.793	& \textbf{30.672}	\\
        500\_60\_5	& 30.763	& \textbf{30.540}	\\
        500\_60\_6	& 30.788	& \textbf{30.597}	\\
        500\_60\_7	& 30.826	& \textbf{30.528}	\\
        500\_60\_8	& 30.837	& \textbf{30.584}	\\
        500\_60\_9	& 30.805	& \textbf{30.645}	\\
        500\_60\_10	& 30.866	& \textbf{30.787}	\\
        600\_20\_1	& 31.372	& 31.600	\\
        600\_20\_2	& 31.397	& 31.753	\\
        600\_20\_3	& 31.429	& 31.670	\\
        600\_20\_4	& 31.487	& 31.759	\\
        600\_20\_5	& 31.407	& 31.769	\\
        600\_20\_6	& 31.696	& 32.035	\\
        600\_20\_7	& 31.527	& 31.951	\\
        600\_20\_8	& 31.523	& 31.701	\\
        600\_20\_9	& 31.532	& 32.052	\\
        600\_20\_10	& 31.107	& 31.361	\\
        600\_40\_1	& 33.683	& \textbf{33.385}	\\
        600\_40\_2	& 33.405	& \textbf{33.237}	\\
        600\_40\_3	& 33.713	& \textbf{33.587}	\\
        600\_40\_4	& 33.584	& \textbf{33.254}	\\
        600\_40\_5	& 33.401	& \textbf{33.220}	\\
        600\_40\_6	& 33.626	& \textbf{33.420}	\\
        600\_40\_7	& 33.545	& \textbf{33.413}	\\
        600\_40\_8	& 33.298	& \textbf{33.078}	\\
        600\_40\_9	& 33.567	& \textbf{33.250}	\\
        600\_40\_10	& 33.473	& \textbf{33.284}	\\
        600\_60\_1	& 35.976	& \textbf{35.920}	\\
        600\_60\_2	& 35.923	& \textbf{35.561}	\\
        600\_60\_3	& 35.917	& \textbf{35.670}	\\
        600\_60\_4	& 36.000	& \textbf{35.640}	\\
        600\_60\_5	& 36.004	& \textbf{35.606}	\\
        600\_60\_6	& 35.943	& \textbf{35.529}	\\
        600\_60\_7	& 35.965	& \textbf{35.717}	\\
        600\_60\_8	& 35.894	& \textbf{35.499}	\\
        600\_60\_9	& 35.987	& \textbf{35.588}	\\
        600\_60\_10	& 35.943	& \textbf{35.563}	\\
        \hline
        \end{tabular}
        \begin{tabular}{|l|l|l|}
            \hline
                & best	& IBS1	\\
            \hline
            700\_20\_1	& 36.388	& 36.916	\\
            700\_20\_2	& 36.316	& 36.676	\\
            700\_20\_3	& 36.519	& 36.971	\\
            700\_20\_4	& 36.380	& 36.619	\\
            700\_20\_5	& 36.556	& 36.956	\\
            700\_20\_6	& 36.645	& 36.927	\\
            700\_20\_7	& 36.597	& 36.912	\\
            700\_20\_8	& 36.492	& 36.790	\\
            700\_20\_9	& 36.315	& 36.634	\\
            700\_20\_10	& 36.386	& 36.839	\\
            700\_40\_1	& 38.767	& \textbf{38.573}	\\
            700\_40\_2	& 38.560	& \textbf{38.316}	\\
            700\_40\_3	& 38.460	& \textbf{38.261}	\\
            700\_40\_4	& 38.597	& \textbf{38.460}	\\
            700\_40\_5	& 38.490	& \textbf{38.339}	\\
            700\_40\_6	& 38.440	& \textbf{38.352}	\\
            700\_40\_7	& 38.355	& \textbf{38.189}	\\
            700\_40\_8	& 38.817	& \textbf{38.778}	\\
            700\_40\_9	& 38.569	& 38.825	\\
            700\_40\_10	& 38.712	& \textbf{38.635}	\\
            700\_60\_1	& 41.192	& \textbf{40.772}	\\
            700\_60\_2	& 41.002	& \textbf{40.664}	\\
            700\_60\_3	& 41.173	& \textbf{40.581}	\\
            700\_60\_4	& 41.120	& \textbf{40.491}	\\
            700\_60\_5	& 41.167	& \textbf{40.641}	\\
            700\_60\_6	& 41.159	& \textbf{40.714}	\\
            700\_60\_7	& 40.734	& \textbf{40.331}	\\
            700\_60\_8	& 41.305	& \textbf{40.830}	\\
            700\_60\_9	& 41.111	& \textbf{40.501}	\\
            700\_60\_10	& 41.186	& \textbf{40.730}	\\
            800\_20\_1	& 41.479	& 41.843	\\
            800\_20\_2	& 41.345	& 41.623	\\
            800\_20\_3	& 41.399	& 41.693	\\
            800\_20\_4	& 41.426	& 42.056	\\
            800\_20\_5	& 41.705	& 41.959	\\
            800\_20\_6	& 41.961	& 42.416	\\
            800\_20\_7	& 41.395	& 41.812	\\
            800\_20\_8	& 41.435	& 42.022	\\
            800\_20\_9	& 41.783	& 42.113	\\
            800\_20\_10	& 41.568	& 41.908	\\
            800\_40\_1	& 43.466	& \textbf{43.261}	\\
            800\_40\_2	& 43.575	& \textbf{43.289}	\\
            800\_40\_3	& 43.596	& \textbf{43.313}	\\
            800\_40\_4	& 43.743	& \textbf{43.491}	\\
            800\_40\_5	& 43.794	& 46.117	\\
            800\_40\_6	& 43.638	& \textbf{43.370}	\\
            800\_40\_7	& 43.484	& \textbf{43.384}	\\
            800\_40\_8	& 43.666	& \textbf{43.469}	\\
            800\_40\_9	& 43.643	& \textbf{43.477}	\\
            800\_40\_10	& 43.630	& \textbf{43.446}	\\
            800\_60\_1	& 46.279	& \textbf{45.680}	\\
            800\_60\_2	& 46.232	& \textbf{45.728}	\\
            800\_60\_3	& 46.258	& \textbf{45.698}	\\
            800\_60\_4	& 46.261	& \textbf{45.696}	\\
            800\_60\_5	& 46.164	& \textbf{45.490}	\\
            800\_60\_6	& 46.288	& \textbf{45.504}	\\
            800\_60\_7	& 46.061	& \textbf{45.600}	\\
            800\_60\_8	& 46.257	& \textbf{45.964}	\\
            800\_60\_9	& 46.279	& \textbf{45.766}	\\
            800\_60\_10	& 46.211	& \textbf{45.383}	\\
            \hline
            \end{tabular}
}    
